Three Dimensional Velocity Measurement Using a Dual Axis Millimeter-Wave Interferometric Radar

In this work, a method for directly measuring target velocity in three dimensions using a dual axis correlation interferometric radar is presented. Recent advances have shown that the measurement of a target's angular velocity is possible by correlating the signals measured at spatially diverse aperture locations. By utilizing multiple orthogonal baselines and using conventional Doppler velocity methods to obtain radial velocity, a full three-dimensional velocity vector can be obtained using only three receive antennas and a single transmitter, without the need for tracking. A $\text{41.8 GHz}$ dual axis interferometric radar with a $7.26\lambda$ antenna baseline is presented along with measurements of a target moving parallel to the plane of the radar array, and of a target moving with components of both radial and tangential velocity. These experiments achieved total velocity root-mean-square errors of $\text{41.01 mm}\cdot\text{s}^{-1}$ ($10.5\%$) for a target moving along a plane parallel to the array, and $\text{45.07 mm}\cdot\text{s}^{-1}$ ($13.5\%$) for a target moving with components of radial and tangential motion relative to the array; estimated trajectory angle RMSEs of $10.42^\circ$ and $5.11^\circ$ were achieved for each experiment respectively.

==> Rev 4.0 - arXiv Documents/acronyms.tex <==
% --- Acronyms ------------------------
\DeclareAcronym{lfm}{
	short = LFM,
	long = linear frequency modulation
}
\DeclareAcronym{prf}{
	short = PRF,
	long = pulse repetition frequency
}
\DeclareAcronym{fmcw}{
	short = FMCW,
	long = frequency modulated continuous-wave
}
\DeclareAcronym{cw}{
	short = CW,
	long = continuous-wave
}
\DeclareAcronym{dbf}{
	short = DBF,
	long = digital beamforming
}
\DeclareAcronym{crlb}{
	short = CRLB,
	long = Cramér-Rao lower bound
}
\DeclareAcronym{dof}{
	short = DoF,
	long = degree of freedom
}
\DeclareAcronym{if}{
	short = IF,
	long = intermediate frequency
}
\DeclareAcronym{adc}{
	short = ADC,
	long = analog to digital converter
}
\DeclareAcronym{fft}{
	short = FFT,
	long = fast Fourier transform,
}
\DeclareAcronym{rmse}{
	short = RMSE,
	long = root-mean-square error
}
\DeclareAcronym{psd}{
	short = PSD,
	long = power spectral density
}

\DeclareAcronym{ni}{
	short = NI,
	long = National Instruments
}

\DeclareAcronym{daq}{
	short = DAQ,
	long = data acquisition
}

\DeclareAcronym{snr}{
	short = SNR,
	long = signal-to-noise ratio
}


\DeclareAcronym{doa}{
	short = DOA,
	long = direction of arrival
}

\DeclareAcronym{adi}{
	short = ADI,
	long = Analog Devices
}

\DeclareAcronym{vco}{
	short = VCO,
	long = voltage-controlled oscillator
}

\DeclareAcronym{lna}{
	short = LNA,
	long = low-noise amplifier
}

\DeclareAcronym{lo}{
	short = LO,
	long = local oscillator
}


\DeclareAcronym{hci}{
	short = HCI,
	long = human-computer interaction
}

\DeclareAcronym{mimo}{
	short = MIMO,
	long = multiple-input multiple-output
}

\DeclareAcronym{simo}{
	short = SIMO,
	long = single-input multiple-output
}

\DeclareAcronym{mmic}{
	short = MMIC,
	long = monolithic microwave integrated circuit
}
